Incremental Learning of Motion Primitives for Pedestrian Trajectory Prediction at Intersections

This paper presents a novel incremental learning algorithm for pedestrian motion prediction, with the ability to improve the learned model over time when data is incrementally available. In this setup, trajectories are modeled as simple segments called motion primitives. Transitions between motion primitives are modeled as Gaussian Processes. When new data is available, the motion primitives learned from the new data are compared with the previous ones by measuring the inner product of the motion primitive vectors. Similar motion primitives and transitions are fused and novel motion primitives are added to capture newly observed behaviors. The proposed approach is tested and compared with other baselines in intersection scenarios where the data is incrementally available either from a single intersection or from multiple intersections with different geometries. In both cases, our method incrementally learns motion patterns and outperforms the offline learning approach in terms of prediction errors. The results also show that the model size in our algorithm grows at a much lower rate than standard incremental learning, where newly learned motion primitives and transitions are simply accumulated over time.

==> discussion.tex <==
\section{DISCUSSION}
This work proposed Similarity-based Incremental Learning Algorithm (SILA) for prediction of pedestrians trajectory when the data is incrementally available in one or across multiple intersections. A new model is learned from new data and the similarity between motion primitives from new and pre-trained models is computed for fusion of two models. The experimental result confirms that SILA is able to incrementally learn and improve the prediction accuracy over the time and outperform batch (off-line) learning in predicting the pedestrian trajectories in intersections, while the learning time is constantly small, which enables SILA for online learning applications. While prediction accuracy of is comparable to standard incremental learning, where the newly learned model are simply accumulated, the model size grows up to \ghcomment{xx} percent slower than standard approach. 

In the future, SILA can be considered as a meta learning approach for learning new motion behaviors. The extension of SILA for multi-agent learning is left for further study.
\ghcomment{time complexity?}
%% quick update enables a rapid adaptationaccording to new information, but old information is forgotten equally quickly.On the other hand, adaption can be performed slowly, in which case old informa-tion is retained longer but the reactivity of the system is decreased. The dilemmabehind this trade-off is usually denoted thestability-plasticity dilemma, which isa well-known constraint for artificial as well as biological learning systems [113].Incremental learning techniques, which adapt learned models to concept driftonly in those regions of the data space where concept drift actually occurs, offera partial remedy to this problem. Many online learning methods alone, albeitdealing with limited resources, are not able to solve this dilemma since theyexhibit a so-calledcatastrophic forgettingbehaviour [44, 45, 108, 103, 132] evenwhen the new data statistics do not invalidate the old ones.One approach to deal with the stability-plasticity dilemma consists in theenhancement of the learning rules by explicit meta-strategies, when and how tolearn.
